HeadRouter: A Training-free Image Editing Framework for MM-DiTs by Adaptively Routing Attention Heads

Diffusion Transformers (DiTs) have exhibited robust capabilities in image generation tasks. However, accurate text-guided image editing for multimodal DiTs (MM-DiTs) still poses a significant challenge. Unlike UNet-based structures that could utilize self/cross-attention maps for semantic editing, MM-DiTs inherently lack support for explicit and consistent incorporated text guidance, resulting in semantic misalignment between the edited results and texts. In this study, we disclose the sensitivity of different attention heads to different image semantics within MM-DiTs and introduce HeadRouter, a training-free image editing framework that edits the source image by adaptively routing the text guidance to different attention heads in MM-DiTs. Furthermore, we present a dual-token refinement module to refine text/image token representations for precise semantic guidance and accurate region expression. Experimental results on multiple benchmarks demonstrate HeadRouter's performance in terms of editing fidelity and image quality.

==> Figures/sup_more.tex <==
\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.97\linewidth]{Images/sup_more.pdf}
 \vspace{-3mm}
  \caption{\textbf{More results generated by our methods.}}
   \vspace{-3mm}
  \label{fig:sup_more}
\end{figure*}

==> Figures/sup_verification_IARouter.tex <==
\begin{figure}[!h]
  \centering
  \includegraphics[width=0.95\linewidth]{Images/sup_verification_IARouter.pdf}
  \vspace{-2mm}
  \caption{\textbf{Verification of the IARouter effectiveness.} }
  \vspace{-4mm}
  \label{fig:sup_verification_IARouter}
\end{figure}

==> Figures/teaser.tex <==
\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.97\linewidth]{Images/teaser.pdf}
  \caption{\textbf{Teasers.}}
  \label{fig:teaser}
\end{figure*}

==> Tables/alignment_ablation.tex <==
\begin{table*}[!th]
\centering
\caption{\textbf{Comparison of cosine similarity between CLIP (for style and prompt) and DINO features (for content) of the generated images and reference style, content, and prompt, respectively}. Our method has the best average score, indicating that our approach successfully customizes the generation of the target content and style while aligning with the prompt.}
\label{tab:alignment_ablation}
\begin{tabular}{c|ccccccc|ccc|c}
\toprule
Methods   &SDEdit &P2P+NTI     &Instruct-Pix2Pix &MasaCrtl &InfEdit &LEDITS++   &RF-Inver &w/o SFR &w/o DTR1    &Ours     \\ \hline
Reference-alignment $(\uparrow)$   &0.5221 &0.4942  &0.4816   &0.5181 &\textbf{0.5319}  &0.5175  &0.5265  &0.5119  &0.5288 \\ \hline
Prompt-alignment $(\uparrow)$     &0.5438 & 0.6092 & 0.6165  &0.6345 &0.6403  &0.5835  &0.6297  &0.6615  &\textbf{0.6754} \\  \hline
Image-quality $(\uparrow)$    &0.3038 & 0.2836 & 0.3156  &0.2778 &0.3319  &0.3971  &0.4046  &0.3908  &\textbf{0.4107} \\ \hline
\textbf{Average} $(\uparrow)$    &0.4566 & 0.4623 & 0.4712  &0.4768 &0.5014  &0.4994  &0.5203  &0.5214  &\textbf{0.5383} \\ \bottomrule
\end{tabular}
\end{table*}
